Exploring Gender Bias in Remote Pair Programming among Software Engineering Students: The twincode Original Study and First External Replication

Context. Software Engineering (SE) has low female representation due to gender bias that men are better at programming. Pair programming (PP) is common in industry and can increase student interest in SE, especially women; but if gender bias affects PP, it may discourage women from joining the field. Objective. We explore gender bias in PP. In a remote setting where students cannot see their peers' gender, we study how perceived productivity, technical competency and collaboration/interaction behaviors of SE students vary by perceived gender of their remote partner. Method. We developed an online PP platform (twincode) with a collaborative editing window and a chat pane. Control group had no gender information about their partner, while treatment group saw a gendered avatar as a man or woman. Avatar gender was swapped between tasks to analyze 45 variables on collaborative coding behavior, chat utterances and questionnaire responses of 46 pairs in original study at the University of Seville and 23 pairs in the replication at the University of California, Berkeley. Results. No significant effect of gender bias treatment or interaction between perceived partner's gender and subject's gender in any variable in original study. In replication, significant effects with moderate to large sizes in four variables within experimental group comparing subjects' actions when partner was male vs female.

==> duran_emse_twincode_2022_04_04_material.tex <==
% ------------------------------------------------------
% File    : duran_emse_twincode_2022_04_05_material.tex
% Content : Participants of the article for EMSE 2022
% Date    : 10/06/2022
% Version : 1.0
% Authors : A. Durán
% ------------------------------------------------------

% ------------------------------------------------------
% Last update: First version (10/06/2022 - Amador)
% Rename and review for journal version. 
% ------------------------------------------------------

%---------------------------------
\subsection{Experimental Material} \label{sec:material}
%---------------------------------

The experimental material \ldots
